MemoCRS: Memory-enhanced Sequential Conversational Recommender Systems with Large Language Models

Conversational recommender systems (CRSs) aim to capture user preferences and provide personalized recommendations through multi-round natural language dialogues. However, most existing CRS models mainly focus on dialogue comprehension and preferences mining from the current dialogue session, overlooking user preferences in historical dialogue sessions. The preferences embedded in the user's historical dialogue sessions and the current session exhibit continuity and sequentiality, and we refer to CRSs with this characteristic as sequential CRSs. In this work, we leverage memory-enhanced LLMs to model the preference continuity, primarily focusing on addressing two key issues: (1) redundancy and noise in historical dialogue sessions, and (2) the cold-start users problem. To this end, we propose a Memory-enhanced Conversational Recommender System Framework with Large Language Models (dubbed MemoCRS) consisting of user-specific memory and general memory. User-specific memory is tailored to each user for their personalized interests and implemented by an entity-based memory bank to refine preferences and retrieve relevant memory, thereby reducing the redundancy and noise of historical sessions. The general memory, encapsulating collaborative knowledge and reasoning guidelines, can provide shared knowledge for users, especially cold-start users. With the two kinds of memory, LLMs are empowered to deliver more precise and tailored recommendations for each user. Extensive experiments on both Chinese and English datasets demonstrate the effectiveness of MemoCRS.

==> body.tex <==

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{imgs/diver_network_structure.pdf}
%     \caption{Overall network structure.}
%     \label{fig:overall_framework}
% \end{figure*}

% \section{Problem Formulation}
%  \wwadd{$x_v$, $\Delta(S)$}Given a set of users $\mathcal U=\{1,\ldots,n_u\}$, a set of items $\mathcal V=\{1,\ldots,n_v\}$, and an initial ranking list $R(u)\in \Pi_L(\mathcal V)$ of $L$ items for users $u\in \mathcal U$, our task is to re-rank $R(u)$ and generate a list of $K$ distinct items $S(u)$ that better satisfies users' preferences and needs, usually $K<L$.
 
%  The probability of the user $u$ is attracted by item $v_k\in S(u)$ is a combination of two terms: a relevance term and a diversity term. The relevance of an item, in our setting, depends on the current item as well as local contexts and influence by other items in the list. The diversity term is the diversity gain in topic coverage, weighted by users' diversified interests towards different topics.
%  \begin{align}
%      \bar a_u(v_k) = &\lambda \phi_u(v_k|S(u))\tag{relevance}\\
%      &+ (1-\lambda)\langle\theta^u, \Delta(v_k|\{v_1,\ldots, v_{k-1}\})\rangle,\tag{diversity}\\\label{eq:diver_attr}
%  \end{align}
 
%   where $\phi_u(v_k|S(u))$ is relevance score of item $v_k$ given the presence of other items in the initial lists, and $\Delta(v_k|\{v_1,\ldots, v_{k-1}\})=c(\{v_1,\ldots, v_{k-1}\}\cup \{v_k\})-c(\{v_1,\ldots, v_{k-1}\})$ is the topic coverage gain by item $v_k$ over the previous $k-1$ items,  $\theta^u=(\theta^u_1,\ldots,\theta^u_m)$ is the personalized topic preferences of a user $u$, which is a distribution over $m$ topics.
 
% \begin{algorithm}[H]
% \caption{\texttt{Diver}}
% \begin{algorithmic}[1]
% \REQUIRE $u,R(u),K,\lambda, \Delta$, $\hat e_u$, $\hat a_u$, $\hat{\theta}^u$
% \ENSURE $S$
% \STATE $S\leftarrow\emptyset$
% \WHILE{$|S|< K$} 
% \STATE $v^*\leftarrow\arg\max_{v\in R\setminus S}P(v|u)+\lambda\tau_u P(v,\bar S|u)$
% \STATE $R\leftarrow R\setminus \{v^*\}$
% \STATE $S\leftarrow S\cup\{v^*\}$
% \ENDWHILE
% \RETURN $S$
% \end{algorithmic} 
% \label{alg:main}
% \end{algorithm}


 
 \section{Proposed Model}
 \subsection{Attractiveness Estimation}
 \subsubsection{Relevance}
 \begin{equation}
     \phi_u(v_k|S(u)) = f_\Phi(x_{v_k}|\{x_{v_1},\ldots,x_{v_K}\}, x_u)
 \end{equation}
 \subsubsection{Personalized Topic Preferences}
 The model takes as input the user positively interacted items grouped by different topics, and outputs the topic preferences $\hat \theta^u$.
 
 \subsection{Termination Estimation}
 \begin{equation}
     \hat e_u = f_\Theta(x_{v_k}|\{x_{v_1},\ldots,x_{v_K}\}, x_u)
 \end{equation}
 
 \subsection{Re-ranking}
 \wwadd{Use the upper bound, Ranking under uncertainty} We select the re-ranked list that maximizes the probability that a user feels satisfied
 \begin{equation}\label{eq:diver_max}
     S(u) = {\arg\max}_{A\in\Pi_K(R(u))}f(A, \hat e_u, \hat a_u).
 \end{equation}
 It can be easily shown that the expected reward is maximized when the attractiveness the items are listed in the same decreasing order of the termination probability.

\subsection{Optimization}
We optimize the lower bound of the log-likelihood of the dependent click model, to push the model to score satisfying items higher than the negative ones,
% \begin{align*}
%     \mathcal L_{lower} =&\sum_{k=1}^K \Big(y_u(v_k)\log\left( \hat{a}_u(v_k)\right)\\
%     + &\left(1- y_u(v_k)\right)\log\left(1-\hat{a}_u(v_k)\right)\Big)\\
%     + &\sum_{k=1}^{K-1}y_u(v_k)\log e_u(k) + \log(1-e_u(k)),\\
% \end{align*}

\begin{align*}
    \mathcal L_{lower} =&\sum_{k=1}^K \Big(y_u(v_k)\log\left( \hat{a}_u(v_k)\right) + \left(1- y_u(v_k)\right)\log\left(1-\hat{a}_u(v_k)\right)\Big)\\
    + &\sum_{k=1}^{K-1}y_u(v_k)\log (1-e_u(k)) + \log(e_u(K)),\\
\end{align*}
\wwadd{this objective function does not work well, need revise}

\section{Theoretical Analysis}
\input{theorem}


\section{Experiments}
\begin{itemize}
    \item (RQ1) How does Diver perform as compared with the state-of-the-art reranking models in terms of utility and diversity?
    \item (RQ2) How well does Diver perform on different scenarios with various importance of diversity?
    \item (RQ3) How well does Diver perform on different initial ranking lists?
    \item (RQ4) How do different hyper-parameter settings (the dimension of hidden states, \wwadd{and others?}) influence the performance of Diver?
    \item (RQ5) How does each designed component (the user history behaviors, the aggregation function) influence the performance of Diver?
\end{itemize}

\subsection{Dataset}
\subsubsection{Taobao}
Taobao data is a dataset consisting of user behavior data retrieved from Taobao\footnote{\url{https://tianchi.aliyun.com/dataset/dataDetail?dataId=649}}, one of the biggest e-commerce platforms in China, with 987,994 users, 4,162,042 items, and 100,150,807 interactions. It contains user behaviors from November 25 to December 3, 2017. We select top 10,000 users with the highest number of interactions, whose data from first 2 days is used to learn personalized topic preferences. And their next 3 days (3-5 days) are selected as training set, and following 3 day(6-8 day) and the last day are validation set and test set, respectively.  We use Gaussian Mixture Models(GMMs) to compute $h_j(v)$, the probability of item $v$ covering topic $j$.

\subsubsection{MovieLens-20M\footnote{\url{https://grouplens.org/datasets/movielens/20m/}}}
This dataset describes free-text tagging activity and 5-star rating for movies from MovieLens\footnote{\url{https://movielens.org/}}, a movie recommendation service. It contains 20000263 ratings and 465564 tag applications across 27278 movies, created by 138493 users between January 09, 1995 and March 31, 2015. We only remain users with more than 200 interactions, then we random shuffle all the remaining records and divide the data set into user profile history, training set, validation set, and test set in the ratio of 2:3:4:1. Given all the movies in MovieLens-20M belong to 20 genres, we use the normalized multi-hot genre vector as the probability of item $v$ covering topic $j$,  $h_j(v)$.

\subsubsection{Huawei Data}
Our algorithms are evaluated on a proprietary dataset obtained from Huawei App store. We use \textit{Gaussian Mixture Models} (GMMs) to compute $h_j(v)$ the probability of item $v$ covering topic $j$. Huawei data has 17 different categories: number of topics $m=17$?

\subsection{Click Feedback}
 \subsubsection{Dependent Click Model}
The system displays an ordered list of $K$ items to the user. The user examines the items in the displayed order and clicks on the attracted items. After an item
is clicked, the user may either be satisfied and leave, or proceed to the next item. The user leaves if all $K$ items have been examined, regardless of whether the user has found any satisfactory item or not.

For each user, the model is parameterized by $K$ \textit{item-dependent attraction probabilities} $\bar w_u\in[0,1]^K$, and $K$ \textit{position-dependent termination probabilities} $\bar e_u\in[0,1]^K$. The user checks the list of items one by one from top to bottom. For each item $v_k$, the user is attracted with probability $\bar a_u(v_k)$. If the user is attracted by $v_k$, then she clicks it and examines the item. The user may be satisfied and leave, which happens with probability $\bar e_u(k)$. The user may also continues to check the next item (which happens with probability $1-\bar e_u(k)$). If all items have been checked and the user has not found any satisfactory item, then the user leaves, unsatisfied.

The probability that a user $u$ is satisfied with list is
\begin{equation}
    f(S, \bar e_u, \bar a_u)=1-\prod_{k=1}^K\left(1-\bar e_u(k)\bar a_u(v_k)\right).
\end{equation}

\subsubsection{Submodular Diverse Model}
Suppose items belongs to $m$ topics, then the topic coverage of a list $c(S)\in[0,1]^m$, is an $m$-dimensional vectors whose $j$-th entry is the coverage of topic $j\in \{1,\ldots,m\}$. We assume $c_j(S)$ is a monotone and submodular function in $S$ for any $j\in \{1,\ldots,m\}$:
\begin{align}
    \forall S\subseteq S' & \subseteq \mathcal V, v\in \mathcal V:  \nonumber\\
    & c_j(S\cup \{v\})\geq c_j(S) \tag{monotonicity}\\
    \text{and}\: & c_j(S\cup \{v\}) - c_j(S) \geq c_j(S'\cup \{v\}) - c_j(S'). \tag{submodularity}
\end{align}
For example, a commonly adopted diverse function is the probabilistic coverage function,
\begin{equation}
    c_j(S) = 1 - \prod_{v\in S}(1-h_j(v)),
\end{equation}
where $h_j(v)$ is the probability of item $v$ covering topic $j$, and $c_j(s)$ is the $j$-th entry of $c(S)$, describing the probability of at least one item the list $S$ covers topic $j$. Clearly, such a function is monotone and submodular in each entry of $c(S)$.

\subsection{Evaluation Metrics}
\wwadd{\begin{itemize}
    \item accuracy-based: ndcg, map, clicks
    \item diversity-based: lntra list similarity, probabilistic coverage diversity
    \item Dependent click models.
\end{itemize}}


\subsection{Baselines}
\begin{itemize}
    \item DLCM
    \item Seq2Slate
    \item PRM
    \item SetRank
    \item MMR (search result diversification re-ranking method)
    \item Xquad (search result diversification re-ranking method)
\end{itemize}

\subsection{Initial Rankers}
\begin{itemize}
    \item \wwadd{DIN}
    \item SVMRank
    \item LambdaMart
    \item Urank (other learning to rank methods)
\end{itemize}

\subsection{Overall Performance}
\wwadd{The utility-diversity tradeoff exists widely.}
\wwadd{Initial ranker is not diversified, focusing a certain popular topics.}

% \begin{table*}[]
% \footnotesize
% \begin{threeparttable}
% \begin{tabular}{cccccc|ccccc}
% \toprule
%               & ndcg@3          & utility@3       & ILS@3           & diversity@3         & satisfaction@3     & ndcg@5          & utility@5       & ILS@5           & diversity@5         & satisfaction@5      \\ \midrule
% initial ranker & 0.2281          & \textbf{0.1657} & 2.7011          & 2.42502314          & 0.07603935          & \textbf{0.3085} & \textbf{0.2691} & 2.2518          & 3.33045927         & \textbf{0.15295046} \\
% prm            & 0.2274          & 0.1632          & 2.7013          & 2.42542491          & 0.07627046          & 0.3076          & 0.2664          & 2.2501          & 3.3302738          & 0.15218162          \\
% diver          & \textbf{0.2284} & 0.165           & \textbf{2.6997} & \textbf{2.42567061} & \textbf{0.07651311} & 0.3084          & 0.266           & \textbf{2.2492} & \textbf{3.3328366} & 0.15114638               \\\bottomrule
% \end{tabular}
% \end{threeparttable}
% \end{table*}

% \begin{table*}[]
% \centering
% \caption{Overall Performance. $\lambda=0.5$}
% \begin{threeparttable}
% \begin{tabular}{lllll|llll}
% \toprule
%           & MRR@5 & utility@5 & div@5 & satis@5 & MRR@10 & utility@10  & div@10 & satis@10 \\\midrule
% Init      &  0.6482 & 1.2334  & 3.0854 & 0.221 & 0.5623 & 1.8755  & 4.221 & 0.1661   \\
% SetRank   &   0.6208 & 1.4593  & 3.1789 & 0.2573 & 0.5564 & 2.1065  & 4.2927 & 0.1835   \\
% % Seq2Slate &  & & & & & & &   \\
% DLCM      &  0.7071 & 1.7284  & 3.2719 & 0.2975 & 0.6755 & 2.4087  & 4.349 & 0.2056  \\
% PRM       &  \textbf{0.7267 }& 1.7893  & 3.1774 & 0.3064 & 0.6992 & 2.4519  & 4.2834 & 0.2083  \\

% \midrule
% MMR       &  0.6713 & 1.1002  & 2.3698 & 0.1992 & 0.545 & 1.8017  & 3.7387 & 0.1616   \\
% DPP       & 0.652 & 1.2564  & \textbf{3.4495} & 0.2247 & 0.5789 & 1.8625  & \textbf{4.4414} & 0.1644   \\\midrule
% Diver & 0.7098 & \textbf{1.8260} & 3.2858 & \textbf{0.3121} & 0.6858 & \textbf{2.5277 }& 4.4167 & \textbf{0.2144} \\
% \bottomrule
% % Diver-seq2seq & & & & & & & & & & \\\bottomrule
% \end{tabular}
% \end{threeparttable}
% \end{table*}

\begin{table*}[]
\centering
\scriptsize
\caption{Overall Performance. $\lambda=0.5$}
\begin{threeparttable}
\begin{tabular}{ccccc|cccc|cccc|cccc}
\toprule
               & \multicolumn{8}{c|}{Taobao}                                                                                                                    & \multicolumn{8}{c}{MovieLens-20M}                                                                                                             \\\cmidrule{2-17}
               & util@5          & ndcg@5          & div@5           & satis@5         & util@10         & ndcg@10         & div@10          & satis@10        & util@5          & ndcg@5          & div@5           & satis@5         & util@10         & ndcg@10         & div@10          & satis@10        \\\midrule
Init           & 1.2432          & 0.4103          & 3.0849          & 0.2227          & 1.8912          & 0.5054          & 4.2208          & 0.1674          & 1.8412          & 0.4936          & 5.6425          & 0.3190          & 2.3379          & 0.5383          & 7.1999          & 0.2743          \\
SetRank        & 1.6935          & 0.4553          & 3.1826          & 0.2925          & 2.2972          & 0.5629          & 4.2621          & 0.1963          & 2.0630          & 0.5185          & 6.2412          & 0.3511          & 2.6291          & 0.5692          & 7.8875          & 0.3032          \\
DLCM           & 1.7284          & 0.4933          & 3.2719          & 0.2975          & 2.4087          & 0.6039          & 4.3490          & 0.2056          & 2.0960          & 0.5438          & 6.5144          & 0.3555          & 2.6540          & 0.5924          & 8.1239          & 0.3055          \\
PRM            & 1.7893          & 0.5041          & 3.1774          & 0.3064          & 2.4519          & 0.6134          & 4.2834          & 0.2083          & 2.0911          & 0.5267          & 6.2818          & 0.3550          & 2.6560          & 0.5775          & 7.8888          & 0.3057          \\
\textbf{Diver} & \textbf{1.8260} & \textbf{0.5065} & \textbf{3.2858} & \textbf{0.3121} & \textbf{2.5277} & \textbf{0.6206} & \textbf{4.4167} & \textbf{0.2144} & \textbf{2.1068} & \textbf{0.5490} & \textbf{6.5634} & \textbf{0.3570} & \textbf{2.6623} & \textbf{0.5975} & \textbf{8.1706} & \textbf{0.3063}  \\\midrule
MMR            & 1.2560          & 0.4100          & 3.2464          & 0.2247          & 1.8938          & 0.5048          & 4.2611          & 0.1674          & 1.8575          & 0.4857          & 5.8207          & 0.3214          & 2.3455          & 0.5280          & 7.3301          & 0.2750          \\
DPP            & 1.3326          & 0.4259          & \underline{4.1645}          & 0.2377          & 1.8732          & 0.5023          & \underline{4.5851}          & 0.1645          & 1.9458          & 0.5065          & 6.4568          & 0.3342          & 2.4378          & 0.5480          & \underline{8.3408}          & 0.2846          \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}


% \begin{table*}[]
% \centering
% \caption{Overall Performance. $\lambda=0.9$}
% \begin{threeparttable}
% \begin{tabular}{lllll|llll}
% \toprule
%           & MRR@5 & utility@5  & div@5 & satis@5 & MRR@10 & utility@10  & div@10 & satis@10 \\\midrule
% Init      &  0.5287 & 1.2594  & 3.0854 & 0.2246 & 0.3835 & 2.1672  & 4.221 & 0.1923 \\
% SetRank   &  0.5417 & 2.2346  & 3.1658 & 0.3707 & 0.4912 & 3.1768  & 4.2632 & 0.2621 \\
% % Seq2Slate &  & & & & & & &   \\
% DLCM      &  0.7251 & 2.5603  & 3.195 & 0.4106 & 0.7028 & 3.4622  & 4.2731 & 0.2797   \\
% PRM       &  0.7627 & 2.5927  & 3.1974 & 0.4144 & 0.7464 & 3.5072  & 4.2738 & 0.2826     \\
% \midrule
% MMR       & 0.5342 & 1.2273  & 2.4744 & 0.2194 & 0.3817 & 2.1325  & 3.4594 & 0.1897   \\
% DPP       & 0.5373 & 1.2226  & \textbf{3.4495} & 0.219 & 0.3902 & 2.1023  & \textbf{4.4414} & 0.1872  \\\midrule
% % Diver   & \textbf{0.7657} & \textbf{2.6760} & 3.1982 & \textbf{0.4253} & \textbf{0.7555} & \textbf{3.5881} & 4.2807 & \textbf{0.2876 }\\
% Diver & 0.7562 & \textbf{2.6357} & 3.2001 & \textbf{0.4203} & 0.7427 & \textbf{3.5691} & \textbf{4.2813} & \textbf{0.2869} \\
% % Diver &  & & & & & & &   \\
% \bottomrule
% % Diver-seq2seq  & & & & & & & & & & \\\bottomrule
% \end{tabular}
% \end{threeparttable}
% \end{table*}

\begin{table*}[]
\centering
\scriptsize
\caption{Overall Performance. $\lambda=0.9$}
\begin{threeparttable}
\begin{tabular}{ccccc|cccc|cccc|cccc}
\toprule
               & \multicolumn{8}{c|}{Taobao}                                                                                                                    & \multicolumn{8}{c}{MovieLens-20M}                                                                                                             \\\cmidrule{2-17}
               & util@5          & ndcg@5          & div@5           & satis@5         & util@10         & ndcg@10         & div@10          & satis@10        & util@5          & ndcg@5          & div@5           & satis@5         & util@10         & ndcg@10         & div@10          & satis@10        \\\midrule
Init           & 1.2698          & 0.3302          & 3.0845          & 0.2264          & 2.1849          & 0.4331          & 4.2207          & 0.1937          & 1.7972          & 0.4067          & 5.6412          & 0.3103          & 2.4889          & 0.4418          & 7.1997          & 0.2871          \\
SetRank        & 2.3785          & 0.6152          & 3.1870          & 0.3893          & 3.3416          & 0.7159          & 4.2706          & 0.2731          & 2.2401          & 0.4820          & 5.8967          & 0.3738          & 3.0700          & 0.5273          & 7.5221          & 0.3428          \\
DLCM           & 2.5603          & 0.6872          & 3.1950          & 0.4106          & 3.4622          & 0.7769          & 4.2731          & 0.2797          & 2.2393          & 0.4871          & 5.8975          & 0.3736          & 3.0700          & 0.5324          & 7.5226          & 0.3428          \\
PRM            & 2.5927          & 0.7001          & 3.1974          & 0.4144          & 3.5072          & 0.7915          & 4.2738          & 0.2826          & 2.2428          & 0.4874          & 5.8957          & 0.3741          & 3.0735          & 0.5325          & 7.5191          & 0.3431          \\
\textbf{Diver} & \textbf{2.6357} & \textbf{0.7090} & \textbf{3.2001} & \textbf{0.4203} & \textbf{3.5691} & \textbf{0.8022} & \textbf{4.2813} & \textbf{0.2869} & \textbf{2.2437} & \textbf{0.4881} & \textbf{5.8995} & \textbf{0.3742} & \textbf{3.0740} & \textbf{0.5329} & \textbf{7.5254} & \textbf{0.3431} \\ \midrule
MMR            & 1.2636          & 0.3264          & 3.2439          & 0.2256          & 2.1824          & 0.4302          & 4.2708          & 0.1937          & 1.8005          & 0.4060          & 5.7282          & 0.3108          & 2.4905          & 0.4415          & 7.2514          & 0.2873          \\
DPP            & 1.2109          & 0.3188          & \underline{4.1641}          & 0.2174          & 2.0838          & 0.4164          & \underline{4.5847}          & 0.1858          & 1.8077          & 0.4052          & \underline{6.4558}          & 0.3119          & 2.4959          & 0.4406          & \underline{8.3398}          & 0.2879          \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}

% \begin{table*}[]
% \centering
% \caption{Overall Performance. $\lambda=1$}
% \begin{threeparttable}
% \begin{tabular}{lllll|llll}
% \toprule
%           & MRR@5 & utility@5  & div@5 & satis@5 & MRR@10 & utility@10  & div@10 & satis@10 \\\midrule
% Init      &  0.5292 & 1.2660  & 3.0854 & 0.2256 & 0.3692 & 2.2402  & 4.221 & 0.1987 \\
% % Seq2Slate &   0.5288 & 1.2762  & 3.0848 & 0.2273 & 0.3693 & 2.2578  & 4.2206 & 0.2002   \\
% SetRank   &   0.5731 & 2.4516  & 3.1898 & 0.3994 & 0.5116 & 3.5506  & 4.2723 & 0.2884  \\
% DLCM      &   0.7509 & 2.7410  & 3.1961 & 0.4327 & 0.731 & 3.7163  & 4.2738 & 0.2966      \\
% PRM       &   \textbf{0.7995} & 2.7718  & 3.1944 & 0.4355 & \textbf{0.7891} & 3.7553  & 4.278 & 0.2993   \\
% \midrule
% MMR       & 0.5292 & 1.2660  & 3.0854 & 0.2256 & 0.3692 & 2.2402  & 4.2210 & 0.1987 \\
% DPP       & 0.5393 & 1.2142  & \textbf{3.4495} & 0.2177 & 0.3747 & 2.1623  & \textbf{4.4414} & 0.1928  \\\midrule
% Diver     & 0.7745 & \textbf{2.8400} & 3.1991 & \textbf{0.4449} & 0.7672 & \textbf{3.8464} & 4.2790 & \textbf{0.3050} \\
% % Diver &  & & & & & & &   \\
% \bottomrule
% % Diver-seq2seq  & & & & & & & & & & \\\bottomrule
% \end{tabular}
% \end{threeparttable}
% \end{table*}


\begin{table*}[]
\centering
\scriptsize
\caption{Overall Performance. $\lambda=1.0$}
\begin{threeparttable}
\begin{tabular}{ccccc|cccc|cccc|cccc}
\toprule
               & \multicolumn{8}{c|}{Taobao}                                                                                                                    & \multicolumn{8}{c}{MovieLens-20M}                                                                                                             \\\cmidrule{2-17}
               & util@5          & ndcg@5          & div@5           & satis@5         & util@10         & ndcg@10         & div@10          & satis@10        & util@5          & ndcg@5          & div@5           & satis@5         & util@10         & ndcg@10         & div@10          & satis@10        \\\midrule
Init           & 1.2761          & 0.3163          & 3.0845          & 0.2273          & 2.2578          & 0.4198          & 4.2204          & 0.2002          & 1.7862                                 & 0.3897                                 & 5.6412                                 & 0.3085                                 & 2.5265                                 & 0.4244                                 & 7.1992                                 & 0.2905                                 \\
SetRank        & 2.5298          & 0.6449          & 3.1922          & 0.4100          & 3.6154          & 0.7465          & 4.2759          & 0.2925          & 2.2823                                 & 0.4989                                 & 5.8110                                 & 0.3793                                 & 3.2359                                 & 0.5432                                 & 7.5369                                 & 0.3505                                 \\
DLCM           & 2.7410          & 0.7375          & 3.1961          & 0.4327          & 3.7163          & 0.8222          & 4.2738          & 0.2966          & 2.2857                                 & 0.5006                                 & 5.7986                                 & 0.3797                                 & 3.3456                                 & 0.5543                                 & 7.6914                                 & 0.3478                                 \\
PRM            & 2.7718          & 0.7517          & 3.1944          & 0.4355          & 3.7553          & 0.8378          & 4.2780          & 0.2993          & 2.2853                                 & 0.5008                                 & 5.8059                                 & 0.3797                                 & 3.1791                                 & 0.5417                                 & 7.4360                                 & 0.3524                                 \\
\textbf{Diver} & \textbf{2.8400} & \textbf{0.7639} & \textbf{3.1991} & \textbf{0.4449} & \textbf{3.8464} & \textbf{0.8511} & \textbf{4.2790} & \textbf{0.3050} & {\color[HTML]{7B7F83} \textbf{2.2854}} & {\color[HTML]{7B7F83} \textbf{0.5018}} & {\color[HTML]{7B7F83} \textbf{5.8081}} & {\color[HTML]{7B7F83} \textbf{0.3797}} & {\color[HTML]{7B7F83} \textbf{3.2894}} & {\color[HTML]{7B7F83} \textbf{0.5483}} & {\color[HTML]{7B7F83} \textbf{7.6129}} & {\color[HTML]{7B7F83} \textbf{0.3492}} \\ \midrule
MMR            & 1.2635          & 0.3127          & 3.2440          & 0.2256          & 2.2521          & 0.4172          & 4.2708          & 0.2000          & 1.7862                                 & 0.3902                                 & 5.6414                                 & 0.3085                                 & 2.5266                                 & 0.4248                                 & 7.1996                                 & 0.2905                                 \\
DPP            & 1.1792          & 0.2990          & \underline{4.1639}          & 0.2121          & 2.1347          & 0.4022          & \underline{4.5848}          & 0.1909          & 1.7733                                 & 0.3890                                 & \underline{6.4559}                                 & 0.3067                                 & 2.5109                                 & 0.4228                                 & \underline{8.3403}                                 & 0.2890                                 \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}

\begin{table*}[]
\centering
\small
\caption{Huawei App Store}
\begin{threeparttable}
\begin{tabular}{ccccccc}
\toprule
               & revenue@3                     & div@3                         & revenue@5                     & div@5                         & revenue@10                    & div@10                        \\\midrule
Init           & 1.7720                        & 0.1075                        & 2.4445                        & 0.1537                        & 3.4300                        & 0.2325                        \\
SetRank        & {\color[HTML]{A5A5A5} 1.6960} & {\color[HTML]{A5A5A5} 0.1071} & {\color[HTML]{A5A5A5} 2.3081} & {\color[HTML]{A5A5A5} 0.1519} & {\color[HTML]{A5A5A5} 3.2902} & {\color[HTML]{A5A5A5} 0.2286} \\
DLCM           & 1.8527                        & 0.1079                        & 2.5292                        & 0.1560                        & 3.5263                        & 0.2381                        \\
PRM            & 1.8708                        & 0.1082                        & 2.5382                        & 0.1556                        & 3.5025                        & 0.2356                        \\
\textbf{Diver} & \textbf{1.9075}               & \textbf{0.1096}               & \textbf{2.6228}               & \textbf{0.1579}               & \textbf{3.5625}               & \textbf{0.2386}               \\\midrule
MMR            & 1.3960                        & 0.1066                        & 2.1156                        & 0.1476                        & 3.2371                        & 0.2260                        \\
DPP            & 1.3686                        & \underline{0.1282}                        & 2.0921                        & \underline{0.2008}                        & 3.2310                        & \underline{0.2905}                        \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}


\begin{figure}[t] %hbt
	\vspace{-0pt}
	\centering
	\includegraphics[width=0.235\textwidth]{imgs/case_dive_hist.pdf}
	\includegraphics[width=0.235\textwidth]{imgs/case_dive_rerank.pdf}
	\vspace{-18pt}
	\caption{The distributions of items for a users with diverse interests. }
	\label{fig:sample}
	\vspace{-10pt}
\end{figure}

\begin{figure}[t] %hbt
	\vspace{-0pt}
	\centering
	\includegraphics[width=0.235\textwidth]{imgs/case_homo_hist.pdf}
	\includegraphics[width=0.235\textwidth]{imgs/case_homo_rerank.pdf}
	\vspace{-18pt}
	\caption{The distributions of items for a users with single interest. }
	\label{fig:sample}
	\vspace{-10pt}
\end{figure}

 \section{Literature Review}
 \subsection{Reranking for Recommender Systems}
 Several existing works have demonstrated the effectiveness of re-ranking by modeling item mutual influences and interactions in the initial ranking lists \cite{dlcm,prm,setrank,feng2021revisit}.
For example, Ai \etal \cite{dlcm} use a recurrent neural network to sequentially encode the top-ranked items with their feature vectors, and learn a local context model to re-rank the top results. Similarly, Zhuang \etal \cite{zhuang2018globally} design a recurrent neural network with an attention mechanism to capture long-distance influences between items.

Inspired by the Transformer architecture \cite{vaswani2017attention} used in machine translation, Pei \etal \cite{prm} propose to use the Transformer to model the mutual influences between items. The Transformer structure uses the self-attention mechanism where the relationship between any two items is reflected with an attention score. Pang \etal \cite{setrank} study the permutation-invariant property of the self-attention blocks in re-ranking. Feng \etal \cite{feng2021revisit} also investigate the permutation influence in re-ranking and generate candidate re-ranking permutations by beam search. Yet all of them overlook users' diversified interests towards the re-ranked lists.


 \subsection{Diversity}
In the context of search result diversification, explicit intent-aware diversity frameworks aim at promoting a hybrid of coverage over explicit aspects of a query and novelty. An early example of such kind of algorithm in information retrieval is the Maximum Marginal Relevance (MMR) re-ranking algorithm~\cite{carbonell1998use}. IA-Select \cite{agrawal2009diversifying} maximizes the probability that the average user finds at least one useful result within the top-$K$ results. PM-2 \cite{dang2012diversity} provides search results that best maintain the overall proportionality of documents belonging to different aspects. The intra-list similarity is calculated in \cite{ziegler2005improving} to diversify the topics in the list. xQuAD \cite{santos2010exploiting} is a probabilistic framework to balance relevance and novelty. However, result diversification in these information retrieval applications focuses on diversifying the search results over topic aspects and does not study users' personal diversified preferences towards the re-ranked lists. \wwadd{DPP NIPS'18}

% \url{https://zhuanlan.zhihu.com/p/72202739}
% calibrated recommendation
% Data-driven experiments on Huawei.
